GRID: Protecting Training Graph from Link Stealing Attacks on GNN Models

Graph neural networks (GNNs) have exhibited superior performance in various classification tasks on graph-structured data. However, they encounter the potential vulnerability from the link stealing attacks, which can infer the presence of a link between two nodes via measuring the similarity of its incident nodes' prediction vectors produced by a GNN model. Such attacks pose severe security and privacy threats to the training graph used in GNN models. In this work, we propose a novel solution, called Graph Link Disguise (GRID), to defend against link stealing attacks with the formal guarantee of GNN model utility for retaining prediction accuracy. The key idea of GRID is to add carefully crafted noises to the nodes' prediction vectors for disguising adjacent nodes as n-hop indirect neighboring nodes. We take into account the graph topology and select only a subset of nodes (called core nodes) covering all links for adding noises, which can avert the noises offset and have the further advantages of reducing both the distortion loss and the computation cost. Our crafted noises can ensure 1) the noisy prediction vectors of any two adjacent nodes have their similarity level like that of two non-adjacent nodes and 2) the model prediction is unchanged to ensure zero utility loss. Extensive experiments on five datasets are conducted to show the effectiveness of our proposed GRID solution against different representative link-stealing attacks under transductive settings and inductive settings respectively, as well as two influence-based attacks. Meanwhile, it achieves a much better privacy-utility trade-off than existing methods when extended to GNNs.

==> Makefile <==
# Makefile for LaTeX document files
# Created by Baochun Li, bli@eecg.toronto.edu, March 30 2001
# Last modified: September 27 2002 

DOCUMENT=main

default: $(DOCUMENT).pdf

$(DOCUMENT).toc: $(DOCUMENT).tex
	pdflatex $(DOCUMENT).tex

$(DOCUMENT).pdf: $(DOCUMENT).toc
	bibtex $(DOCUMENT)
	pdflatex $(DOCUMENT).tex
	pdflatex $(DOCUMENT).tex

#--------------------------------------------------
# $(DOCUMENT).ps: $(DOCUMENT).dvi
# 	dvips -t letter -Ppdf -G0 -o $@ $<
# 
# $(DOCUMENT).pdf: $(DOCUMENT).ps
# 	cat $(DOCUMENT).ps | ps2pdf - > $(DOCUMENT).pdf 
#-------------------------------------------------- 

all: $(DOCUMENT).pdf

clean:
	rm -rf *.aux $(DOCUMENT).log $(DOCUMENT).toc \
     $(DOCUMENT).bbl $(DOCUMENT).blg *.bak \
		 $(DOCUMENT).out \

     #$(DOCUMENT).pdf \


==> Related.tex <==
\section{Related Work}
\label{sec:related}


\subsection{Membership Inference Attack}


Originated from the field of biology for inferring genome information~\cite{homer2008resolving,hagestedt2020membership,hagestedt2019mbeacon}, membership inference attack (MIA) has recently become a popular concept in the machine learning area for inferring if a given data was used to train a machine learning (ML) model. 
The first study of MIA in the ML area was proposed in~\cite{shokri2017membership}, with two key designs: 1)  training multiple shadow models to fit the output patterns of a target model and 2) building a classifier trained for learning the difference between prediction vectors of training and of non-member data. 
Plentiful follow-up research has been introduced to improve such original designs or apply them to different learning algorithms/models~\cite{salem2019ml,li2021membership,leino2020stolen, choquette2021label,liu2021encodermi,salem2020updates,nasr2019comprehensive,sablayrolles2019white,song2021systematic,song2019privacy,hidano2021transmia,carlini2021extracting,song2020information,li2021membership2}, such as contrastive learning, online learning, transfer learning, federated learning, natural language domains, among others. 
Some studies~\cite{he2021node,wu2021adapting,olatunji2021membership} also extended MIA into the context of GNNs, for inferring the individual node samples in the training graphs, i.e., node attributes. 
The main clue for the success of these MIA lies in that the prediction vectors outputted by a trained model will be overfitted, thus able to exhibit the membership patterns. 


Recently, the first comprehensive link inference attack toward GNN models was proposed in~\cite{he2021stealing} to steal the link-presence information of the training graph. 
Different from aforementioned node-level inference attacks which measure the overfitting for conducting MIA, link stealing attacks leverage the characteristic of GNN model which aggregates information for each node from its neighboring nodes, causing the high similarity between prediction vectors of linked nodes (i.e., neighboring nodes). 
Hence, an attacker can measure the similarity between prediction vectors of two query nodes to determine if a link exists between them. 
A subsequent  work~\cite{wu2024link} then extended this idea on the inductive GNN models.
On the other hand, \cite{wu2022linkteller,meng2023devil} proposed the influence-based link-stealing attacks which leverages the observation that two nodes are more likely to be linked if changing the features of one node significantly influences the prediction results of the other node due to the message-passing mechanism. 
%The essence of this attack is also to measure the similarity of prediction vectors of two querying nodes for link inference. 



\subsection{Defense for MIA}
\label{subsec:defense}
After realizing the potential risk of MIA, some defense approaches have been proposed to counter such attacks, and they can be grouped into three categories: 
1) employing differential privacy principles~\cite{shokri2015privacy,abadi2016deep,wang2017differentially,yu2019differentially,wu2022linkteller,sajadmanesh2023gap}; 2) using adversarial learning methods~\cite{carlini2017towards,moosavi2017universal,papernot2016limitations}; and 3) preventing prediction result overfitting~\cite{li2021membership2,nasr2018machine,salem2019ml,song2021systematic}.
Such three categories of solutions usually inevitably disrupt the training process of a target model, thus incurring considerable model accuracy degradation.
%For example, the solutions proposed in~\cite{shokri2017membership,srivastava2014dropout,nasr2018machine}  for preventing model overfitting have to disrupt the training process of a target model for reducing the overfitting of prediction vectors. 
For example, the L2-Regularizer~\cite{shokri2017membership} and Min-Max Game~\cite{nasr2018machine} added additional terms to the objective functions for overfitting prevention, inevitably degrading the accuracy of the target model (i.e., incurring utility loss).
Besides, the differential privacy~\cite{mulle2015privacy, wu2022linkteller, sajadmanesh2022gap} can be applied for protecting GNN against the link steal attacks, but still suffering the considerable utility loss as presented in \cite{wu2022linkteller, sajadmanesh2022gap}.
%Therefore, these approaches ensure model defense at the cost of model performance. 
In conclusion, solutions aimed at reducing overfitting or those that introduce perturbations, prove inefficient in defending against link stealing attacks on GNN models while maintaining a guarantee of utility preservation. 
In other words, current methods struggle to strike a balance between protecting the model from link stealing attacks and preserving the model's prediction performance.

On the other hand, the MemGuard~\cite{jia2019memguard} was proposed to defend against membership inference attacks with the formal model utility loss guarantee.
Instead of intervening in the training process, MemGuard adds noise vectors to the prediction vectors of a trained model.
By distorting these prediction vectors, membership patterns become obscured, making it difficult for an attacker to infer if a querying sample belongs to the member of the training dataset. 
Moreover, the utility loss of the prediction vector is kept within bounds by moderating the intensity of the noise vectors.
However, MemGuard's protection of the GNN model is limited to the node-level, preventing only the inference of node attributions, as the noise is computed to hide the relationship of the individual node prediction vector and its attributes.
It is insufficient to defend against the link stealing attack, which has to focus on the relationship of prediction vectors between any nodes pairs.
A new methodology is therefore required, which considers graph topology and node relationships when introducing noise for each node. 


